SMT 2.0: A Surrogate Modeling Toolbox with a focus on Hierarchical and Mixed Variables Gaussian Processes

The Surrogate Modeling Toolbox (SMT) is an open-source Python package that offers a collection of surrogate modeling methods, sampling techniques, and a set of sample problems. This paper presents SMT 2.0, a major new release of SMT that introduces significant upgrades and new features to the toolbox. This release adds the capability to handle mixed-variable surrogate models and hierarchical variables. These types of variables are becoming increasingly important in several surrogate modeling applications. SMT 2.0 also improves SMT by extending sampling methods, adding new surrogate models, and computing variance and kernel derivatives for Kriging. This release also includes new functions to handle noisy and use multifidelity data. To the best of our knowledge, SMT 2.0 is the first open-source surrogate library to propose surrogate models for hierarchical and mixed inputs. This open-source software is distributed under the New BSD license.

==> MLP_tikz.tex <==
\begin{tikzpicture}

% N:node, 1:layer, (u,c,b) : up, center, below

% input-layer (first layer) %
\node [draw, circle, minimum size=0.75cm] (N1c) at (0,0) {\large $\alpha_i^{(in)}$};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N1c), label={\hspace{-0.5cm} \vspace{0.5cm} \Large Input layer}] (N1u) {\large $\alpha_1^{(in)}$};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N1c)] (N1b) {\large $\alpha_p^{(in)}$};

\node [at=($(N1c)!0.5!(N1b)$)] {\Huge \vdots} ;
\node [at=($(N1c)!0.5!(N1u)$)] {\Huge \vdots} ;
%----------%


% 2nd layer %
%\node [draw, circle, minimum size=1cm, at=($(N1c)+(2.5,0)$)] (N2c) {};
%\node [draw, circle, minimum size=1cm, at=($(N1u)+(2.5,-1)$)] (N2u) {};
%\node [draw, circle, minimum size=1cm, at=($(N1b)+(2.5,+1)$)] (N2b) {};

\node [draw, circle, minimum size=0.75cm, xshift=3.5cm, yshift=0cm, at=(N1c)] (N2c) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N2c)] (N2u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N2c)] (N2b) {};

\node [at=($(N2c)!0.5!(N2b)$)] {\Huge \vdots} ;
\node [at=($(N2c)!0.5!(N2u)$)] {\Huge \vdots} ;
%----------%

% 3nd layer %
\node [draw, circle, minimum size=0.75cm, xshift=2.5cm, yshift=0cm, at=(N2c)] (N3c) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N3c)] (N3u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N3c)] (N3b) {};


\node [at=($(N3c)!0.5!(N3b)$)] {\Huge \vdots} ;
\node [at=($(N3c)!0.5!(N3u)$)] {\Huge \vdots} ;
%----------%


% n-1 layer %
\node [draw, circle, minimum size=0.75cm, xshift=5cm, yshift=0cm, at=(N3c)] (N6c) {}; %computed from N3c
% boxed

\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N6c)] (N6u) {};

\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N6c)] (N6b) {};

\node [at=($(N6c)!0.5!(N6b)$)] {\Huge \vdots} ;
\node [at=($(N6c)!0.5!(N6u)$)] {\Huge \vdots} ;
%----------%



% n layer %
\node [draw, circle, minimum size=0.75cm, xshift=2.5cm, yshift=0cm, at=(N6c)] (N7c) {}; 
\node [draw, fill=black!25, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N7c)] (N7u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N7c)] (N7b) {};

% Three nodes
\node [at=($(N7c)!0.43!(N7b)$)] {\Huge \vdots} ;
\node [at=($(N7c)!0.57!(N7u)$)] {\Huge \vdots} ;

% Two nodes
%\node [at=($(N7u)!0.42!(N7b)$)] {\Huge \vdots} ;
%----------%


% output  %
\node [draw, circle, minimum size=1cm, xshift=3cm, yshift=0cm, at=(N7c), label={ \Large Output}] (N8c) {\large $\psi \left(\alpha^{(in)}\right )$}; %computed from N3c

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N7c)--(N8c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N7u)--(N8c);
\draw[ -{Stealth[length=2mm, width=1.5mm]}] (N7b)--(N8c);
%----------%

% First fake layer
\node [ circle, minimum size=0.75cm, at=($(N3c)!.33!(N6c)$)] (N4c) {};
\node [ circle, minimum size=0.75cm, at=($(N3u)!.33!(N6u)$)] (N4u) {};
\node [ circle, minimum size=0.75cm, at=($(N3b)!.33!(N6b)$)] (N4b) {};

%% 2nd fake%%%
\node [ circle, minimum size=1cm, at=($(N3c)!.66!(N6c)$)] (N5c) {}; 
\node [ circle, minimum size=1cm, at=($(N3u)!.66!(N6u)$)] (N5u) {};
\node [ circle, minimum size=1cm, at=($(N3b)!.66!(N6b)$)] (N5b) {};





%------------------------arretes ---------------------%

% input-to-2nd %
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2b);
%----------%


% 2nd-to-3rd %
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3b);
%----------%


% between 3rd layer and 1st fake
\draw[ - ] (N3c) -- ($(N3c)!.66!(N4c)$); %longer
\draw[ - ] (N3c) -- ($(N3c)!.33!(N4u)$);
\draw[ - ] (N3c) -- ($(N3c)!.33!(N4b)$);

\draw[ - ] (N3u)-- ($(N3u)!.33!(N4c)$);
\draw[ - ] (N3u)-- ($(N3u)!.66!(N4u)$); %longer
\draw[ - ] (N3u)-- ($(N3u)!.25!(N4b)$); % shorter

\draw[ - ] (N3b)-- ($(N3b)!.33!(N4c)$);
\draw[ - ] (N3b)-- ($(N3b)!.25!(N4u)$); %shorter
\draw[ - ] (N3b)-- ($(N3b)!.66!(N4b)$); %longer
%------------------------%

% between 1st-fake and 2nd-fake
\node [at=($(N4c)!0.5!(N5c)$)] {\large \dots } ;
\node [at=($(N4u)!0.5!(N5u)$), rotate=160] {\large \dots } ;
\node [at=($(N4b)!0.5!(N5b)$), rotate=20] {\large \dots } ;
%-----------------%

% between 2nd-fake and n-1
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.5!(N6c)$)--(N6c); 
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.66!(N6u)$)--(N6u);
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.66!(N6b)$)--(N6b);

\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.75!(N6c)$)--(N6c);
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.5!(N6u)$)--(N6u); 
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.8!(N6b)$)--(N6b); % fix

\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.75!(N6c)$)--(N6c);
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.8!(N6u)$)--(N6u); % fix
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.5!(N6b)$)--(N6b); 
%----------------%


% (n-1)-to-(n) %
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6c)--(N7c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6c)--(N7u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6c)--(N7b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6u)--(N7c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6u)--(N7u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6u)--(N7b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6b)--(N7c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6b)--(N7u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6b)--(N7b);
%----------%



%-------------------------------------%
% Trapeze : 4 nodes connected
\node [circle, minimum size=1cm] (T1u) at ($(N2u)-(0.8,-0.8)$)  {};
\node [circle, minimum size=1cm] (T1b) at ($(N2b)-(0.8,0.8)$)  {};
\node [circle, minimum size=1cm] (T2u) at ($(N7u)+(0.8,0.8)$)  {};
\node [circle, minimum size=1cm] (T2b) at ($(N7b)+(0.8,-0.8)$)  {};
% left
\draw[dotted, line width= 0.4mm] ($(T1u)+(0,0)$)--($(T1b)+(0,0)$);
% right
\draw[dotted, line width= 0.4mm] ($(T2u)+(0,0)$)--($(T2b)+(0,0)$);

% upper
%\getangle(T1u)(T2u)a;
\draw[dotted, line width= 0.4mm] ($(T1u)+(0,0)$)--($(T2u)+(0,0)$) node[midway, above, black, %rotate=\anglea
]{\Large Hidden layers $l$} ;

% lower
\draw[dotted, line width= 0.4mm] ($(T1b)+(0,0)$)--($(T2b)+(0,0)$);
%-------------------------------------%


%curly brack for units in a layer
\draw [decorate, decoration = {calligraphic brace,raise=15pt, mirror, amplitude=14pt}, line width = 0.4mm ] ($(N6u)-(0.5,-0.6)$) --  ($(N6b)-(0.5,0.6)$); 

%
\draw[->] ($(N5c)+(0,0)$) -- (7.5, -5) node[inner sep=8pt, at end, yshift=-0.5cm] {\Large $n_{l-1}$} ;


% Boxed
\node [draw, minimum size=0.85cm, line width=0.5mm, at=(N7u)] (N7U) {};

\node [draw, minimum height=4.5cm, minimum width=12.5cm, xshift=2.5cm, yshift=6cm, line width=0.3mm, at=(N7U)] (box) {}; %%%%%%%

\draw[->, inner sep=5pt] (N7U.north) .. controls +(down:0cm) and +(right:0cm) .. (box.south);

\node (boxC) [draw, circle, minimum size=0.85cm, at=(box.west), xshift=2.5cm] {$\alpha_{2}^{(l-1)}$}  ;

\node (boxCC) [ minimum size=0.85cm, at=(box.west), xshift=0.75cm] {\Large$n_{l-1}$}  ;

\node (boxT) [draw, circle, minimum size=0.85cm, at=(boxC), yshift=1.5cm] {$\alpha_{1}^{(l-1)}$}  ;
\node (boxB) [ circle, minimum size=0.85cm, at=(boxC), yshift=-1.5cm] { \vspace{-1cm} \Large \vdots }  ;
\draw [decorate, decoration = {calligraphic brace,raise=15pt, mirror, amplitude=14pt}, line width = 0.4mm ] ($(boxT)-(0.2,-0.6)$) --  ($(boxB)-(0.2,0.6)$) ;

%\node (boxScal) [draw, minimum size=0.85cm, at=(boxC), xshift=3.25cm, label={Scalar product}] {$w^{\top} \cdot \alpha^{(l-1)}$}  ;

\node (boxScal) [draw, minimum size=0.85cm, at=(boxC), xshift=3.25cm, label={Scalar product}] { 
$   \sum \limits_{i=1}^{n_{l-1}} w_i \alpha_i^{(l-1)} $
}  ;

\draw[->] (boxT) -- (boxScal) node[midway, above, black]{$w_{1}$};
\draw[->] (boxC) -- (boxScal) node[midway, above, black]{$w_{2}$};



%---Activation func---%
%label={Act. function}
\node (boxAct) [draw, minimum size=0.85cm, at=(boxScal), xshift=3.25cm, label={Activation function}] {
\begin{tikzpicture}
        \begin{axis}[axis lines=center, width=3.5cm, axis x line shift=1cm, height=3.5cm,
         yticklabels={,,},
         xticklabels={,,}
         ]
        \addplot[color=black]{1/(1+exp(-x))-2};
        \end{axis}
        \end{tikzpicture}
}  ;
%------%

\draw [->] (boxScal) -- (boxAct);

\node (nodeRed) [draw, circle, minimum size=0.85cm, fill=black!25, at=(boxAct), xshift=2.5cm] {$\alpha_{1}^{(l)}$};

\draw [->] (boxAct) -- (nodeRed);



\end{tikzpicture}

==> archi.tex <==
\tikzstyle{abstract}=[rectangle, draw=black, rounded corners, anchor=north]
\tikzstyle{myarrow}=[->, >=open triangle 90, thick]
\tikzstyle{line}=[-, thick]

\begin{tikzpicture}[node distance=1cm, thick, scale=0.6, every node/.style={scale=0.8}]
\node (SMT) [abstract, rectangle split, rectangle split parts=2,text width=3.8cm,rectangle split part fill={blue!50,blue!10}]
{\textbf{SMT}
\nodepart{second}+ problems\\ + sampling\_methods\\ + surrogate\_models};
\node (AuxNode01) [text width=4cm, right=of SMT] {};
\node (problems) [abstract, rectangle split, rectangle split parts=2, below=of SMT,text width=2.7cm,rectangle split part fill={blue!50,blue!10}] {\textbf{problems::\\Problem}
\nodepart{second}+ \_\_call\_\_()\\\# \_evaluate()};
\node (sampling) [abstract, rectangle split, rectangle split parts=2, left=of problems,text width=4.15cm,rectangle split part fill={blue!50,blue!10}]
{\textbf{sampling\_methods::\\SamplingMethod}
\nodepart{second}+ \_\_call\_\_()\\\# \_compute()};
\node (surrogate) [abstract, rectangle split, rectangle split parts=2, below=of AuxNode01,text width=5.7cm,rectangle split part fill={blue!50,blue!10}]
{\textbf{surrogate\_models::\\SurrogateModel}
\nodepart{second}+ set\_training\_values()\\+ update\_training\_values()\\+ set\_training\_derivatives()\\+ update\_training\_derivatives()\\+ predict\_derivatives()\\+ predict\_output\_derivatives()\\+ predict\_variances()\\+ predict\_values()\\+ train()\\\# \_predict\_derivatives()\\\# \_predict\_output\_derivatives()\\\# \_predict\_values()\\\# \_predict\_variances()\\\# \_train()};
\draw[myarrow] (SMT) -| (sampling.north);
\draw[myarrow] (SMT) -- (problems.north);
\draw[myarrow] (SMT) -| (surrogate.north);
\end{tikzpicture}


==> canti.tex <==
\vspace{-5pt}
\captionsetup{justification=raggedright,singlelinecheck=false}
\subfloat[Bending problem]{
\begin{tikzpicture}
    \hspace{-3pt}
    %the points
    \point{origin}{-0.75}{-0.25};
    \point{begin}{0}{0};
    \point{end}{5}{0};
    \point{end_bot}{4.99}{-0.9};
    \point{end_up}{5}{0.5};
    %the beam
    \beam{2}{begin}{end};
    %the support
    \support{3}{begin}[-90];
    %the load
    \load{1}{end}[90]   ;
    %the inscription of the load
 %   \notation{1}{origin}{0};
    \notation{1}{end_up}{$F=50kN$};

     \draw[<->] (end) -- (end_bot) node[midway, right] {$\delta$} ;
     \draw[<->] (0,0.5) -- (5,0.5) node[midway, above] {L};
     
    %the deflection curves
    \draw
      [-, ultra thick] (begin) .. controls (1.5, +.01) and (2.5, -.15) .. (4.93, -0.9)
      [-, ultra thick] (begin) .. controls (1.5, +.01) and (2.5, -.2) .. (4.85, -1.5)
      [-, ultra thick] (begin) .. controls (1.5, +.01) and (2.5, -.4)   .. (4.78, -1.9);
  \end{tikzpicture}
\label{fig:beam}   
}
%\raggedright
%\hfill
\subfloat[Possible cross-section shapes.]{
\centering
\begin{tikzpicture}
\hspace{-50pt}

%%%%%
\tstar{0.25}{0.5}{6}{0}{thick,fill=yellow}
\tstar{0.14}{0.28}{6}{0}{thick,fill=white}

\tstar{0.25}{0.5}{6}{0}{thick,fill=yellow,xshift=-1.2cm}
\tstar{0.08}{0.16}{6}{0}{thick,fill=white,xshift=-1.2cm}

\tstar{0.25}{0.5}{6}{0}{thick,fill=yellow,xshift=-2.4cm}

%%%%%
\def\pos{1.2}
\fill[black] (\pos-0.24,-0.5) -- (\pos-0.24,0.5) -- (\pos+0.24,0.5)  -- (\pos+0.24,-0.5)   -- cycle ;
\fill[black] (\pos-0.5,-0.5) -- (\pos-0.5,-0.18) -- (\pos+0.5,-0.18)  -- (\pos+0.5,-0.5)   -- cycle ; 
\fill[black] (\pos-0.5,0.18) -- (\pos-0.5,0.5) -- (\pos+0.5,0.5)  -- (\pos+0.5,0.18)   -- cycle ;  

\def\pos{2.4}
\fill[black] (\pos-0.19,-0.5) -- (\pos-0.19,0.5) -- (\pos+0.19,0.5)  -- (\pos+0.19,-0.5)   -- cycle ;
\fill[black] (\pos-0.5,-0.5) -- (\pos-0.5,-0.25) -- (\pos+0.5,-0.25)  -- (\pos+0.5,-0.5)   -- cycle ; 
\fill[black] (\pos-0.5,0.25) -- (\pos-0.5,0.5) -- (\pos+0.5,0.5)  -- (\pos+0.5,0.25)   -- cycle ;  

\def\pos{3.6}
\fill[black] (\pos-0.14,-0.5) -- (\pos-0.14,0.5) -- (\pos+0.14,0.5)  -- (\pos+0.14,-0.5)   -- cycle ;
\fill[black] (\pos-0.5,-0.5) -- (\pos-0.5,-0.32) -- (\pos+0.5,-0.32)  -- (\pos+0.5,-0.5)   -- cycle ; 
\fill[black] (\pos-0.5,0.32) -- (\pos-0.5,0.5) -- (\pos+0.5,0.5)  -- (\pos+0.5,0.32)   -- cycle ;  

\vspace{1.2cm}

%%%%%
\fill[green,even odd rule] (0,-1.2) circle (0.5) (0,-1.2) circle (0.33);
\draw (0,-1.2) circle (0.5) ;
\draw (0,-1.2) circle (0.33) 
; 
\fill[green,even odd rule] (-1.2,-1.2) circle (0.5)(-1.2,-1.2) circle (0.17);
\draw (-1.2,-1.2) circle (0.5) ;
\draw (-1.2,-1.2) circle (0.17) 
; 
\fill[green,even odd rule] (-2.4,-1.2) circle (0.5) ;
\draw (-2.4,-1.2) circle (0.5) ;

%%%%%
\def\pos{1.2}
\fill[blue,even odd rule]  (\pos-0.5,-1.7) -- (\pos-0.5,-0.7) -- (\pos+0.5,-0.7) -- (\pos+0.5,-1.7) -- cycle ;

\def\pos{2.4}
\fill[blue,even odd rule]  (\pos-0.5,-1.7) -- (\pos-0.5,-0.7) -- (\pos+0.5,-0.7) -- (\pos+0.5,-1.7) -- cycle   (\pos-0.25,-1.45) -- (\pos-0.25,-0.95) -- (\pos+0.25,-0.95) -- (\pos+0.25,-1.45) -- cycle ;

\def\pos{3.6}
\fill[blue,even odd rule]  (\pos-0.5,-1.7) -- (\pos-0.5,-0.7) -- (\pos+0.5,-0.7) -- (\pos+0.5,-1.7) -- cycle   (\pos-0.35,-1.55) -- (\pos-0.35,-0.85) -- (\pos+0.35,-0.85) -- (\pos+0.35,-1.55) -- cycle ;
  \end{tikzpicture}
  \label{fig:beam_shape}    
}

==> func.tex <==
\vspace{3pt}
\begin{forest}
      for tree={
        font= \small \ttfamily,
        grow'=0,
        child anchor=west,
        parent anchor=south,
        anchor=west,
        calign=first,
        inner xsep=10pt,
        inner ysep = -3pt,
        edge path={
          \noexpand\path [draw, \forestoption{edge}]
          (!u.south west) +(7.5pt,0) |- (.child anchor)  \forestoption{edge label};
        },
        % style for your file node 
        file/.style={edge path={\noexpand\path [draw, \forestoption{edge}]
          (!u.south west) +(7.5pt,0) |- (.child anchor) \forestoption{edge label};},
          inner xsep=2pt, inner ysep=-3pt ,font=\footnotesize \ttfamily
                     },
        before typesetting nodes={
          if n=1
            {insert before={[,phantom]}}
            {}
        },
        fit=band,
        before computing xy={l=15pt},
      }  
    [ \   \normalsize \texttt{SMT 2.0}
     % [config
     % ]
      [ \textcolor{blue}{Sampling methods}
        [Random, file
        ]      
        [Full Factorial, file
        ]
        [ Latin Hypercube Sampling \textcolor{Orchid}{(Nested LHS and Extended LHS)}, file
        ]
      ]
      [ \textcolor{blue}{Problems}
        [Aircraft wing weight, file
        ]      
        [Robot arm position, file
        ]  
        [Water flow through a borehole, file
        ]   
        [Low frequency torsion vibration, file
        ]    
        [Welded beam shear stress, file
        ]  
        [ \textcolor{Orchid}{Mixed integer cantilever beam}, file
        ]
        [ \textcolor{Orchid}{Hierarchical neural network}, file
        ]      
      ]
      [ \textcolor{blue}{Surrogate modeling methods}
        [ RBF: Radial Basis Functions, file
        ]
        [IDW: Inverse-Distance Weighting, file
        ]
        [RMTS: Regularized Minimal-energy Tensor-product Splines, file
        ]
         [LS: Least-Squares approximation, file
        ]      
         [QP: Quadratic Polynomial approximation,  file
        ]
        [Kriging based models,  file
            [Continuous kernels,  file]
            [\textcolor{Orchid}{Hierarchical kernels},  file]
            [\textcolor{Orchid}{Categorical kernels},  file]
            %    [Kriging: Gaussian Process interpolation,  file]
             %   [KPLS: Kriging with Partial Least Squares,  file]
            %    [KPLSK: Kriging with Partial Least Squares+Kriging,  file]
           %     [GEKPLS: Gradient-Enhanced Kriging with Partial Least Squares,  file]
        ]
        [\textcolor{Orchid}{GENN: Gradient-Enhanced Neural Network},  file ]
         [ \textcolor{Orchid}{MGP: Marginal Gaussian Process},  file ]
      ]
      [ \textcolor{blue}{Applications}
          [   Mixture of experts (MOE) , file]
          [  Variable-fidelity modeling (VFM) , file]
          [  Multi-fidelity Kriging (MFK) , file]
         [    \textcolor{Orchid}{ Multi-fidelity KPLS (MFKPLS)} , file]
         [    \textcolor{Orchid}{ Multi-fidelity KPLSK (MFKPLSK)} , file]
         [   Efficient Global Optimization (EGO) , file]
         [  \textcolor{Orchid}{ Mixed-Integer and hierarchical usage surrogates}, file]
      ]
        [ \textcolor{blue}{Interactive notebooks}
          [  SMT tutorial for surrogate modeling, file]
          [  \textcolor{Orchid}{  Noisy Gaussian process (Kriging) }, file]
          [ \textcolor{Orchid}{Multi-fidelity Gaussian process (with or without noise)} , file]
         [  \textcolor{Orchid}{ Gaussian process trajectory Sampling} , file]
         [ \textcolor{Orchid}{ Bayesian optimization to solve unconstrained problems} , file]
         [ \textcolor{Orchid}{ Mixed \& hierarchical Kriging and optimization}, file]
        [ \textcolor{Orchid}{SMT 2.0 Advancements and hierarchical variables}, file]

      ]
    ]
 \end{forest}

==> name.tex <==
\begin{tikzpicture}

% N:node, 1:layer, (u,c,b) : up, center, below

% input-layer (first layer) %
\node [draw, circle, minimum size=0.75cm] (N1c) at (0,0) {\large $\nu_i^{(in)}$};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3cm, at=(N1c), label={\hspace{-0.5cm} \vspace{0.5cm} \Large Input layer}] (N1u) {\large $\nu_1^{(in)}$};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3cm, at=(N1c)] (N1b) {\large $\nu_p^{(in)}$};

\node [at=($(N1c)!0.5!(N1b)$)] {\Huge \vdots} ;
\node [at=($(N1c)!0.5!(N1u)$)] {\Huge \vdots} ;
%----------%


% 2nd layer %
%\node [draw, circle, minimum size=1cm, at=($(N1c)+(2.5,0)$)] (N2c) {};
%\node [draw, circle, minimum size=1cm, at=($(N1u)+(2.5,-1)$)] (N2u) {};
%\node [draw, circle, minimum size=1cm, at=($(N1b)+(2.5,+1)$)] (N2b) {};

\node [draw, circle, minimum size=0.75cm, xshift=3.5cm, yshift=0cm, at=(N1c)] (N2c) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=4.75cm, at=(N2c)] (N2u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-4.75cm, at=(N2c)] (N2b) {};

\node [at=($(N2c)!0.5!(N2b)$)] {\Huge \vdots} ;
\node [at=($(N2c)!0.5!(N2u)$)] {\Huge \vdots} ;
%----------%

% 3nd layer %
\node [draw, circle, minimum size=0.75cm, xshift=2.5cm, yshift=0cm, at=(N2c)] (N3c) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=3.75cm, at=(N3c)] (N3u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-3.75cm, at=(N3c)] (N3b) {};


\node [at=($(N3c)!0.5!(N3b)$)] {\Huge \vdots} ;
\node [at=($(N3c)!0.5!(N3u)$)] {\Huge \vdots} ;
%----------%


% n-1 layer %
\node [draw, circle, minimum size=0.75cm, xshift=5cm, yshift=0cm, at=(N3c)] (N6c) {}; %computed from N3c
% boxed

\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=1.75cm, at=(N6c)] (N6u) {};



\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-1.75cm, at=(N6c)] (N6b) {};

\node [at=($(N6c)!0.5!(N6b)$)] {\Huge \vdots} ;
\node [at=($(N6c)!0.5!(N6u)$)] {\Huge \vdots} ;
%----------%



% n layer %
\node [ circle, minimum size=0.75cm, xshift=2.5cm, yshift=0cm, at=(N6c)] (N7c) {}; 
\node [draw, fill=black!25, circle, minimum size=0.75cm, xshift=0cm, yshift=0.75cm, at=(N7c)] (N7u) {};
\node [draw, circle, minimum size=0.75cm, xshift=0cm, yshift=-0.75cm, at=(N7c)] (N7b) {};

% Three nodes
%\node [at=($(N7c)!0.43!(N7b)$)] {\Huge \vdots} ;
%\node [at=($(N7c)!0.57!(N7u)$)] {\Huge \vdots} ;

% Two nodes
\node [at=($(N7u)!0.42!(N7b)$)] {\Huge \vdots} ;
%----------%


% output  %
\node [draw, circle, minimum size=1cm, xshift=3cm, yshift=0cm, at=(N7c), label={ \Large Output}] (N8c) {\large $\hat{h} \left(\nu^{(in)}\right )$}; %computed from N3c

%\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N7c)--(N8c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N7u)--(N8c);
\draw[ -{Stealth[length=2mm, width=1.5mm]}] (N7b)--(N8c);
%----------%

% First fake layer
\node [ circle, minimum size=0.75cm, at=($(N3c)!.33!(N6c)$)] (N4c) {};
\node [ circle, minimum size=0.75cm, at=($(N3u)!.33!(N6u)$)] (N4u) {};
\node [ circle, minimum size=0.75cm, at=($(N3b)!.33!(N6b)$)] (N4b) {};

%% 2nd fake%%%
\node [ circle, minimum size=1cm, at=($(N3c)!.66!(N6c)$)] (N5c) {}; 
\node [ circle, minimum size=1cm, at=($(N3u)!.66!(N6u)$)] (N5u) {};
\node [ circle, minimum size=1cm, at=($(N3b)!.66!(N6b)$)] (N5b) {};





%------------------------arretes ---------------------%

% input-to-2nd %
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1c)--(N2b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1u)--(N2b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N1b)--(N2b);
%----------%


% 2nd-to-3rd %
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2c)--(N3b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2u)--(N3b);

\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N2b)--(N3b);
%----------%


% between 3rd layer and 1st fake
\draw[ - ] (N3c) -- ($(N3c)!.66!(N4c)$); %longer
\draw[ - ] (N3c) -- ($(N3c)!.33!(N4u)$);
\draw[ - ] (N3c) -- ($(N3c)!.33!(N4b)$);

\draw[ - ] (N3u)-- ($(N3u)!.33!(N4c)$);
\draw[ - ] (N3u)-- ($(N3u)!.66!(N4u)$); %longer
\draw[ - ] (N3u)-- ($(N3u)!.25!(N4b)$); % shorter

\draw[ - ] (N3b)-- ($(N3b)!.33!(N4c)$);
\draw[ - ] (N3b)-- ($(N3b)!.25!(N4u)$); %shorter
\draw[ - ] (N3b)-- ($(N3b)!.66!(N4b)$); %longer
%------------------------%

% between 1st-fake and 2nd-fake
\node [at=($(N4c)!0.5!(N5c)$)] {\large \dots } ;
\node [at=($(N4u)!0.5!(N5u)$), rotate=160] {\large \dots } ;
\node [at=($(N4b)!0.5!(N5b)$), rotate=20] {\large \dots } ;
%-----------------%

% between 2nd-fake and n-1
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.5!(N6c)$)--(N6c); 
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.66!(N6u)$)--(N6u);
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5c)!.66!(N6b)$)--(N6b);

\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.75!(N6c)$)--(N6c);
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.5!(N6u)$)--(N6u); 
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5u)!.8!(N6b)$)--(N6b); % fix

\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.75!(N6c)$)--(N6c);
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.8!(N6u)$)--(N6u); % fix
\draw[ -{Stealth[length=2mm, width=1.5mm]}  ] ($(N5b)!.5!(N6b)$)--(N6b); 
%----------------%


% (n-1)-to-(n) %
%\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6c)--(N7c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6c)--(N7u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6c)--(N7b);

%\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6u)--(N7c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6u)--(N7u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6u)--(N7b);

%\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6b)--(N7c);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6b)--(N7u);
\draw[ -{Stealth[length=2mm, width=1.5mm]} ] (N6b)--(N7b);
%----------%



%-------------------------------------%
% Trapeze : 4 nodes connected
\node [circle, minimum size=1cm] (T1u) at ($(N2u)-(1,-1)$)  {};
\node [circle, minimum size=1cm] (T1b) at ($(N2b)-(1,1)$)  {};
\node [circle, minimum size=1cm] (T2u) at ($(N7u)+(1,0.5)$)  {};
\node [circle, minimum size=1cm] (T2b) at ($(N7b)+(1,-0.5)$)  {};
% left
\draw[dotted, line width= 0.4mm] ($(T1u)+(0,0)$)--($(T1b)+(0,0)$);
% right
\draw[dotted, line width= 0.4mm] ($(T2u)+(0,0)$)--($(T2b)+(0,0)$);

% upper
%\getangle(T1u)(T2u)a;
\draw[dotted, line width= 0.4mm] ($(T1u)+(0,0)$)--($(T2u)+(0,0)$) node[midway, above, black, %rotate=\anglea
]{\Large Hidden layers $l$} ;

% lower
\draw[dotted, line width= 0.4mm] ($(T1b)+(0,0)$)--($(T2b)+(0,0)$);
%-------------------------------------%


%curly brack for units in a layer
\draw [decorate, decoration = {calligraphic brace,raise=15pt, mirror, amplitude=14pt}, line width = 0.4mm ] ($(N6u)-(0.5,-0.6)$) --  ($(N6b)-(0.5,0.6)$); 

%
\draw[->] ($(N5c)+(0,0)$) -- (7.5, -5) node[inner sep=8pt, at end, yshift=-0.5cm] {\Large $n_{l-1}$} ;


% Boxed
\node [draw, minimum size=0.85cm, line width=0.5mm, at=(N7u)] (N7U) {};

\node [draw, minimum height=4.5cm, minimum width=12.5cm, xshift=2.5cm, yshift=6cm, line width=0.3mm, at=(N7U)] (box) {}; %%%%%%%

\draw[->, inner sep=5pt] (N7U.north) .. controls +(down:0cm) and +(right:0cm) .. (box.south);

\node (boxC) [draw, circle, minimum size=0.85cm, at=(box.west), xshift=2.5cm] {$\nu_{2}^{(l-1)}$}  ;

\node (boxCC) [ minimum size=0.85cm, at=(box.west), xshift=0.75cm] {\Large$n_{l-1}$}  ;

\node (boxT) [draw, circle, minimum size=0.85cm, at=(boxC), yshift=1.5cm] {$\nu_{1}^{(l-1)}$}  ;
\node (boxB) [ circle, minimum size=0.85cm, at=(boxC), yshift=-1.5cm] { \vspace{-1cm} \Large \vdots }  ;
\draw [decorate, decoration = {calligraphic brace,raise=15pt, mirror, amplitude=14pt}, line width = 0.4mm ] ($(boxT)-(0.2,-0.6)$) --  ($(boxB)-(0.2,0.6)$) ;

%\node (boxScal) [draw, minimum size=0.85cm, at=(boxC), xshift=3.25cm, label={Scalar product}] {$w^{\top} \cdot \nu^{(l-1)}$}  ;

\node (boxScal) [draw, minimum size=0.85cm, at=(boxC), xshift=3.25cm, label={Scalar product}] { 
$   \sum \limits_{i=1}^{n_{l-1}} w_i \nu_i^{(l-1)} $
}  ;

\draw[->] (boxT) -- (boxScal) node[midway, above, black]{$w_{1}$};
\draw[->] (boxC) -- (boxScal) node[midway, above, black]{$w_{2}$};



%---Activation func---%
%label={Act. function}
\node (boxAct) [draw, minimum size=0.85cm, at=(boxScal), xshift=3.25cm, label={Activation function}] {
\begin{tikzpicture}
        \begin{axis}[axis lines=center, width=3.5cm, axis x line shift=1cm, height=3.5cm,
         yticklabels={,,},
         xticklabels={,,}
         ]
        \addplot[color=black]{1/(1+exp(-x))-2};
        \end{axis}
        \end{tikzpicture}
}  ;
%------%

\draw [->] (boxScal) -- (boxAct);

\node (nodeRed) [draw, circle, minimum size=0.85cm, fill=black!25, at=(boxAct), xshift=2.5cm] {$\nu_{1}^{(l)}$};

\draw [->] (boxAct) -- (nodeRed);



\end{tikzpicture}

==> variable_roles.tex <==
\begin{tikzpicture}
\node(1)[label={}, draw, circle]
at (0,0) 
{\begin{tabular}{c}
Meta (dimensional) \\
Component \\
$x_{\meta}$
\end{tabular}}  ;

\node(2)[label={}, xshift=-5cm, yshift=-1.5cm, at=(1), draw, circle]
{\begin{tabular}{c}
Neutral \\
Component \\
$x_{\neutral}$
\end{tabular}
}
;


\node(3)[label={Decreed}, circle, xshift=5cm, yshift=-2cm, at=(1), draw]
{\begin{tabular}{cc}
  Included  &    Excluded \\
  component &    component \\
  $x_{\decreed}$ &   $\overline{x_{\decreed}}$
\end{tabular}
};

\draw[dotted, line width=0.5mm] (5,0.6)--(5,-4.6);

\draw[->] (1)--(3);


\end{tikzpicture}
